Robust Spatiotemporal Fusion of Satellite Images: A Constrained Convex Optimization Approach

This paper proposes a novel spatiotemporal (ST) fusion framework for satellite images, named Robust Optimization-based Spatiotemporal Fusion (ROSTF). ST fusion is a promising approach to resolve a trade-off between the temporal and spatial resolution of satellite images. Although many ST fusion methods have been proposed, most of them are not designed to explicitly account for noise in observed images, despite the inevitable influence of noise caused by the measurement equipment and environment. Our ROSTF addresses this challenge by formulating noise removal and ST fusion as a unified optimization problem. Specifically, first, we define observation models for satellite images possibly contaminated with random noise, outliers, and/or missing values, and then introduce certain assumptions that would naturally hold between the observed images and the target high-resolution image. Then, based on these models and assumptions, we formulate the fusion problem as a constrained optimization problem and develop an efficient algorithm based on a preconditioned primal-dual splitting method for solving the problem. The performance of ROSTF was verified using simulated and real data. The results show that ROSTF performs comparably to several state-of-the-art ST fusion methods in noiseless cases and outperforms them in noisy cases.

==> Experiments/AblationStudy/ablationstudy.tex <==
\input{Experiments/AblationStudy/without_denoising_metrics}
\input{Experiments/AblationStudy/without_denoising_figure}
\input{Experiments/AblationStudy/average_convergence_iterations_and_performance_metrics}
\input{Experiments/AblationStudy/compare_convergence_figure}
\input{Experiments/AblationStudy/without_12constraint_figure}

\subsection{Ablation Study}
\label{ssec: ablation study}
\textcolor{blue}{
Before comparing ROSTF with state-of-the-art methods, we conduct ablation study to measure the influence of the following key components:}
\begin{itemize}
    \item \textcolor{blue}{The mechanism for denoising the reference HR image, i.e., the first regularization term $\|\D\tilHr\|_{1,2}$ and the third, fourth, sixth, and seventh constraints, $\twonorm{\Hr - (\tilHr + \tilshr)}\leq\varepsilon_{h}$, $\twonorm{\Lr - (\S\B\tilHr + \tilslr)}\leq\varepsilon_{l}$, $\onenorm{\tilshr} \leq \eta_h$, $\onenorm{\tilslr} \leq \eta_l$.}
    
    \item \textcolor{blue}{The first constraint, $\|\D\tilHr-\D\tilHt\|_{p} \leq \alpha$, to encourage the land structure, i.e. the edges, of the reference and target HR images to be similar based on Assumption~i). Hereafter, the constraint is referred to Edge Constraint.}

    \item \textcolor{blue}{The second constraint, $\left| c_{b}- \mathbf{1}^{\top}[\widetilde{\mathbf{h}}_{t}]_{b}/{N_{h}}\right| \leq \beta_{b} \, (b = 1, \ldots, B)$, which is designed based on Assumption~ii), so that the estimated target HR image has a similar average brightness as the target LR image. Hereafter, the constraint is referred to Brightness Constraint.}
\end{itemize}

\textcolor{blue}{
We tested ROSTF with each of the above three components removed. The hyperparameters in each optimization problem and the stopping criterion of each P-PDS-based algorithm to solve it were set as in the original ROSTF. On the other hand, the stepsizes in each algorithm were set as the values computed according to the operator-norm-based design method of variable-wise diagonal preconditioning in (\ref{eq: P-PDS stepsizes calculation}).
}

\subsubsection{The Denoising Mechanism}
\textcolor{blue}{
First, we measure the effectiveness of the denoising mechanism of ROSTF by comparing ROSTF with and without this denoising mechanism. The optimization problem of ROSTF without the denoising mechanism is formulated as
\begin{align}
	\min_{\substack{\tilHr,\tilslt}} \:
	& \|\mathbf{D}\tilHt\|_{1,2} \nonumber\\ 
	\mathrm{s.t.} \:
	& \begin{cases}
        \pnorm{\D\Hr - \D\tilHt} \leq \alpha, \\
        \left| c_{b}- \mathbf{1}^{\top}[\widetilde{\mathbf{h}}_{t}]_{b}/{N_{h}}\right| \leq \beta_{b} \, (b = 1, \ldots, B), \\
	\twonorm{\Lt - (\S\B\tilHt + \tilslt)}\leq\varepsilon_{l},\\
        \onenorm{\tilslt} \leq \eta_l.
	\end{cases}
\label{eq: our ST fusion}
\end{align}
Since the objective function contains only one regularization term for $\tilHt$, no balancing parameter is needed. Also, note that the first constraint based on Assumption~i) is different from the original ROSTF because this optimization problem has no variable $\tilHr$.
}

\textcolor{blue}{
Table~\ref{table: without denoising} shows the average RMSE, SAM, MSSIM, and CC results for each noise case. In the noisy cases, i.e. Case2, Case3, and Case4, as expected, ROSTF without the denoising mechanism performs significantly worse than the original ROSTF due to the direct effect of noise. This shows that the denoising mechanism works effectively to make ROSTF robust to noise. On the other hand, we newly found that in the noiseless case, i.e., Case1, ROSTF without the denoising mechanism achieves slightly better fusion results than the original one. This result indicates that in noiseless cases, the observed HR image $\Hr$ can be used as the reference as it is, and there is no need to estimate $\tilHr$. Furthermore, by removing the variable $\tilHr$, ROSTF does not need the reference LR image $\Lr$ as input in the above optimization problem. Thus, fortunately, if noiseless images can be observed, ROSTF can be applied in situations where only two input images are available, a reference HR image and a target LR image. This result, although unexpected, strengthens our work. We would like to thank you for your helpful comment. 
}

\textcolor{blue}{
Fig.~\ref{fig: without denoising} shows the fusion results of ROSTF-1 without the denoising mechanism for the Site1 simulated data. It can also be visually seen that in Case1, ROSTF-1 without the denoising mechanism obtains a good result based on only two input images. On the other hand, in Case2, Case3, and Case4, the results of ROSTF without the denoising mechanism are contaminated by noise. This is because Edge Constraint copies not only the true edge or spatial structure but also the noise in the reference HR image to the estimated target HR image. The results of this ablation study confirm that the denoising mechanism plays an effective role in avoiding such noise effects.
}

\subsubsection{The Constraints Based on Assumptions}
\textcolor{blue}{
Next, we move on to the ablation studies about the two constraints based on Assumption~i) and Assumption~ii), Edge Constraint and Brightness Constraint. The effectiveness of these constraints is verified in terms of convergence speed and fusion performance.
}

\textcolor{blue}{
Table~\ref{table: convergence iterations} shows, for all the situations, the average number of iterations spent before the algorithms stopped and the average performance results. Note that this number of iterations is not necessarily the number required to meet the stopping criteria, since the algorithms stop after the maximum number of iterations 50000 even if the stopping criteria are not met. The original ROSTF performed best with the fewest number of iterations on average, indicating that both of the two constraints contribute to achieving higher fusion performance with fewer iterations. }

% Therefore, these constraints are essential components for ROSTF to be a practical ST fusion method.
\textcolor{blue}{
Fig.~\ref{fig: convergence results} shows the transition of the objective function values and the PSNRs for the original ROSTF-2, ROSTF-2 without Edge Constraint, and ROSTF-2 without Brightness Constraint in the experiment on the Site1 simulated data. ROSTF-2 without Edge Constraint did not meet thr stopping criterion until 50000 iterations. This can be considered because the solution space of the optimization problem without Edge Constraint was too large to find the optimal solution. This suggests that Edge Constraint has the effect of making the solution space moderately small and speeding up convergence. On the other hand, ROSTF-2 without Brightness Constraint converges faster than ROSTF-2 without Edge Constraint, but shows unstable behavior, especially in the early iterations. This may be because the variable $\tilHt$ is no longer updated as a primal variable when Brightness Constraint is removed. The update equation corresponding to Brightness Constraint in Algorithm~1 is implemented as the only update equation for the primal variable $\tilHt$. On the other hand, the update equations corresponding to the other components for $\tilHt$ update the dual variables $\mathbf{z}_2$, $\mathbf{z}_3$ and $\mathbf{z}_6$. Directly updating the primal variable leads to faster convergence of the algorithm and more stable behavior than updating the primal variable via the update of the dual variables. By introducing Brightness Constraint, the variable $\tilHt$ is updated directly as the primal variable, which improves convergence speed and stability.}

\textcolor{blue}{Fig.~\ref{fig: without 12const results} visually compares the original ROSTF-2 with ROSTF-2 without these constraints. The image estimated by ROSTF-2 without Edge Constraint loses spatial structure, and ROSTF-2 without Brightness Constraint outputs an incorrect brightness image. On the other hand, the original ROSTF-2 estimates brightness close to that of Ground-truth while still preserving spatial structure, indicating that both constraints work effectively.}

